Coarse-to-Fine 3D Keyframe Transporter

Recent advances in Keyframe Imitation Learning (IL) have enabled learning-based agents to solve a diverse range of manipulation tasks. However, most approaches ignore the rich symmetries in the problem setting and, as a consequence, are sample-inefficient. This work identifies and utilizes the bi-equivariant symmetry within Keyframe IL to design a policy that generalizes to transformations of both the workspace and the objects grasped by the gripper. We make two main contributions: First, we analyze the bi-equivariance properties of the keyframe action scheme and propose a Keyframe Transporter derived from the Transporter Networks, which evaluates actions using cross-correlation between the features of the grasped object and the features of the scene. Second, we propose a computationally efficient coarse-to-fine SE(3) action evaluation scheme for reasoning the intertwined translation and rotation action. The resulting method outperforms strong Keyframe IL baselines by an average of >10% on a wide range of simulation tasks, and by an average of 55% in 4 physical experiments.

==> table/ablation.tex <==

% \begin{table*}[h!]
\begin{table}
\centering
\scriptsize
\begin{tabular}{lccccccccccccccccccccc}
\toprule
                    & avg.          & task SR      & GPU              & SGD                \\
Method              & SR $\uparrow$ &STD $\downarrow$& mem $\downarrow$ & time $\downarrow$ \\ \midrule

Ours                & 83            & $\pm14$         & 11GB              & 0.7s              \\
no coarse-to-fine \footnotemark &26 & $\pm27$         & 12GB              & 2.2s              \\
no cross, C2F, seg  & 39            & $\pm27$         & 16GB              & 0.9s              \\
no augmentation     & 77            & $\pm13$         & 11GB              & 0.7s              \\
no segmentation     & 80            & $\pm22$         & 11GB              & 0.7s              \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study} on 9 RLBench tasks shows the importance of each component of our method, i.e., keyframe action through cross-correlation, coarse-to-fine action inference, and in-hand segmentation. \underline{avg. SR} shows the success rate averaged over 9 tasks. \underline{task SR STD} shows the standard deviation of the success rate over 9 tasks. \underline{GPU mem} and \underline{SGD time} show the GPU memory consumption and time for 1 SGD step during training. For details on each task, please see Appendix.\ref{app:ablation}.}

\label{table:ablation}
\end{table}


==> table/rlbench18.tex <==
\begin{table}
\centering
\scriptsize
\begin{tabular}{ccccc}
\toprule
       & \multicolumn{2}{c}{avg.}           & GPU               & SGD                   \\
       & \multicolumn{2}{c}{SR$\uparrow$}   & mem $\downarrow$  & time $\downarrow$     \\ \rule{0pt}{3ex} 
Method & 10 & 100                           & (GB)              & (s)    \\ \midrule
Ours  & 65 & 73                           & 11              & 0.7          \\
RVT   & 62 & 61                           & 13              & 0.5      \\
PerAct & 43 & 44                          & 13              & 0.8        \\
C2FARM & 35 & 44                          & 2               & 0.1      \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Average success rate (\%) over 18 RLBench tasks.}  All baselines are trained on single-task, single-variation setups. Training with $10$ demos, ours achieves a similar performance to the best baseline that is trained with $\times 10$ more demos. Training with $100$ demos, ours outperforms the best baseline by $>10\%$. For more details, plase see Appendix.\ref{app:multi}.}

\label{table:rlbench18}
\end{table}
